Seis2Rock: A Data-Driven Approach to Direct Petrophysical Inversion of Pre-Stack Seismic Data

The inversion of petrophysical parameters from seismic data represents a fundamental step in the process of characterizing the subsurface. We propose a novel, data-driven approach named Seis2Rock that utilizes optimal basis functions learned from well log information to directly link band-limited petrophysical reflectivities to pre-stack seismic data. Seis2Rock is composed of two stages: training and inference. During training, a set of optimal basis functions are identified by performing singular value decomposition on one or more synthetic AVO gathers created from measured or rock-physics synthesized elastic well-logs. In inference, seismic pre-stack data are first projected into a set of band-limited petrophysical properties using the previously computed basis functions; this is followed by regularized post-stack seismic inversion of the individual properties. In this work, we apply the Seis2Rock methodology to a synthetic dataset based on the Smeaheia reservoir model and the open Volve field dataset. Numerical results reveal the ability of the proposed method in recovering accurate porosity, shale content, and water saturation models. Finally, the proposed methodology is applied in the context of reservoir monitoring to invert time-lapse, pre-stack seismic data for water saturation changes.

==> Sections/07_Codes.tex <==
\section{Code Availability}
The code repository of this work can be found at \href{https://github.com/DeepWave-KAUST/Seis2Rock}{https://github.com/DeepWave-KAUST/Seis2Rock}

==> Sections/09_Acronyms.tex <==
\makeglossaries
\newacronym{ccs}{CCS}{Carbon Capture and Storage}
\newacronym{avo}{AVO}{Amplitude Variation with Offset}
\newacronym{svd}{SVD}{Singular Value Decomposition}
\newacronym{optavo}{OptAVO}{Optimal linear AVO Approximation}
\newacronym{pem}{PEM}{Petro-Elastic Modeling}
\newacronym{seis2rock}{Seis2Rock}{Rock-physics AVO inversion framework}
\newacronym{RPM}{RPM}{Rock Physics Model}
\newacronym{ADMM}{ADMM}{Alternating Direction Method of Multipliers}




==> Sections/10_Symbols.tex <==
\makenomenclature

%Rock-physics modelling part
\nomenclature{\(r\)}{physical coefficients or reflectivities}
\nomenclature{\(r_{\phi}\)}{Porosity reflectivity}
\nomenclature{\(r_{V_{sh}}\)}{Shale content reflectivity}
\nomenclature{\(r_{S_w}\)}{Water saturation reflectivity}
\nomenclature{\(\phi\)}{Porosity}
\nomenclature{\(V_{sh}\)}{Shale content}
\nomenclature{\(S_w\)}{Water saturation}
\nomenclature{\(K_{min}\)}{Bulk modulus of the mineral/rock}
\nomenclature{\(\mu_{min}\)}{Shear modulus of the mineral/rock}
\nomenclature{\(\mu_{sat}\)}{Shear modulus of the saturated rock}
\nomenclature{\(K_{dry}\)}{Effective bulk modulus}
\nomenclature{\(\mu_{dry}\)}{Effective shear modulus}
\nomenclature{\(P\)}{Pressure}
\nomenclature{\(C\)}{Coordination number}
\nomenclature{\(\nu_{min}\)}{Poisson ratio of the mineral/rock}
\nomenclature{\(K_{fl}\)}{Bulk modulus of the fluid mix}
\nomenclature{\(\rho_{fl}\)}{Density of the fluid mix}
\nomenclature{\(\rho_{min}\)}{Density of the mineral/rock}
\nomenclature{\(V_p\)}{Compressional wave velocity}
\nomenclature{\(V_s\)}{Shear wave velocity}
\nomenclature{\(g\)}{Non-linear rock-physics model of choice}
\nomenclature{\(\xi\)}{Set of hyper-parameters for the rock-physics modeling.}
\nomenclature{\(T\)}{Temperature}

%Inverse problem
\nomenclature{\(N_t\)}{Number of samples in the time/depth axis}
\nomenclature{\(N_{\theta}\)}{Number of angle gathers}
\nomenclature{\(\mathbf{\widetilde m}\)}{Chosen dictionary of petrophysical paramters}
\nomenclature{\(\mathbf{\widetilde m_b}\)}{Chosen dictionary of the background petrophysical paramters}
\nomenclature{\(\mathbf{\widetilde d}\)}{Modeled seismic gather of size ${N_{\theta} \times N_t}$}
\nomenclature{\(\mathbf{\widetilde d_b}\)}{Modeled background seismic gather of size ${N_{\theta} \times N_t}$}
\nomenclature{\(\mathbf{F}\)}{Matrix of eigenvectors of size $N_{\theta} \times N_t$}
\nomenclature{\(\mathbf{V}\)}{Matrix of eigenvectors of size $N_{\theta} \times N_t$}
\nomenclature{\(\boldsymbol\Lambda\)}{Matrix of Eigenvalues embedded in the diagonal of size $N_t \times N_t$}
\nomenclature{\(\mathbf{C}\)}{Matrix of optimal coefficients}
\nomenclature{\(p\)}{Subset of basis functions}
\nomenclature{\(\mathbf{C_p}\)}{Matrix of optimal coefficients taking $p$ basis functions}
\nomenclature{\(\mathbf{F_p}\)}{Matrix of eigenvectors (basis functions) taking $p$ basis functions}
\nomenclature{\(\mathbf{D}\)}{Pre-stack seismic gather}
\nomenclature{\(\mathbf{D_b}\)}{Pre-stack background synthetic seismic gather}
\nomenclature{\(\mathbf{B}\)}{Petrophysical parameters, one per petrophysical property}
\nomenclature{\(\mathbf{W}\)}{Wavelet operator}
\nomenclature{\(\mathbf{T}\)}{Time-derivative operator}
\nomenclature{\(\pmb{\widetilde{R}}\)}{Matrix of petrophysical reflectivities}
\nomenclature{\(n_m\)}{number of petrophysical parameters to invert (i.e., porosity, shale content, and water saturation.}






